Real-Time Online Stock Forecasting Utilizing Integrated Quantitative and Qualitative Analysis

The application of Machine learning to finance has become a familiar approach, even more so in stock market forecasting. The stock market is highly volatile, and huge amounts of data are generated every minute globally. The extraction of effective intelligence from this data is of critical importance. However, a collaboration of numerical stock data with qualitative text data can be a challenging task. In this work, we accomplish this by providing an unprecedented, publicly available dataset with technical and fundamental data and sentiment that we gathered from news archives, TV news captions, radio transcripts, tweets, daily financial newspapers, etc. The text data entries used for sentiment extraction total more than 1.4 Million. The dataset consists of daily entries from January 2018 to December 2022 for eight companies representing diverse industrial sectors and the Dow Jones Industrial Average (DJIA) as a whole. Holistic Fundamental and Technical data is provided training ready for Model learning and deployment. Most importantly, the data generated could be used for incremental online learning with real-time data points retrieved daily since no stagnant data was utilized. All the data was retired from APIs or self-designed robust information retrieval technologies with extremely low latency and zero monetary cost. These adaptable technologies facilitate data extraction for any stock. Moreover, the utilization of Spearman's rank correlation over real-time data, linking stock returns with sentiment analysis has produced noteworthy results for the DJIA and the eight other stocks, achieving accuracy levels surpassing 60%. The dataset is made available at https://github.com/batking24/Huge-Stock-Dataset.

==> Sections/Abstract.tex <==
\begin{abstract} 

\noindent { 
\begin{abstract}
The application of Machine learning to finance has become a familiar approach, even more so in stock market forecasting. The stock market is highly volatile and huge amounts of data are generated every minute globally. The extraction of effective intelligence from this data is of critical importance. However, a collaboration of numerical stock data with qualitative text data can be a challenging task. In this work, we accomplish this and provide an unprecedented, publicly available dataset with technical and fundamental data, sentiment that we gathered from News Archives, TV news captions, Radio Transcripts, Tweets, Daily financial newspapers, etc. The text data entries used for sentiment extraction total more than 1.4 Million. The dataset consists of daily entries from January 2018 to December 2022 for 8 companies representing diverse industrial sectors and the Dow Jones Industrial Average (DJIA) as a whole. Holistic Fundamental and Technical data is provided training ready for Model learning and deployment. Most importantly, the data generated could be used for Incremental online learning with real-time data points retrieved daily since there was no stagnant data utilized. All the data was retired from APIs or self-designed robust information retrieval technologies. Moreover, the utilization of  Spearman's rank correlation over real-time data, linking stock returns with sentiment analysis has produced noteworthy results for the DJIA achieving accuracy levels surpassing 60\%. The dataset is made available at \href{https://github.com/batking24/Huge-Stock-Dataset}{Github}.
\end{abstract}


\end{abstract}




==> Sections/Method.tex <==
\section{Method}


==> Sections/techincal_table.tex <==
% \documentclass[11pt,letterpaper,twoside]{article}
\usepackage[total={6in,10in},left=1.5in,top=0.5in,includehead,includefoot]{geometry}
\usepackage{tabularx}
% \begin{document}
\begin{table}
	\centering
	\renewcommand{\arraystretch}{1.5}
	\begin{tabularx}{\textwidth}{|X|l|p{4cm}|l|}
	\hline
	\multicolumn{1}{|c|}{\textsf{Sections}}
	& \multicolumn{1}{c|}{\textsf{Questions}}
	& \multicolumn{1}{c|}{\textsf{Exercises}}
	& \multicolumn{1}{c|}{\textsf{Problems}}
	\\ \hline
	% Chapter 1 :
	Read the whole chapter, except sections 1.5, which is optional. & 2, 3, 14 & 1, 5, 7, 8, 11, 12, 15, 17, 20, 21, 32 & 1, 5, 6, 8, 13
	\\ \hline
	% Chapter 2 :
	2.1 to 2.10 & 1, 8 & 1, 3, 5, 9, 10, 14, 17, 19, 20, 23, 27, 29, 32, 35, 36, 38 & 4
	\\ \hline
	% Chapter 3 :
	3.1 to 3.5 & 4, 10 & 1, 3, 4, 5 & 3, 6, 9
	\\ \hline
	\end{tabularx}
\end{table}
% \end{document}

\begin{verbatim}
\newcounter{foo}
\setcounter{foo}{5}    
\end{verbatim}
\newcounter{foo}
\setcounter{foo}{5} 
Lists are easy to create:
\begin{itemize}
  \item List entries start with the \verb|\item| command.
  \item Individual entries are indicated with a black dot, a so-called bullet.
  \item The text in the entries may be of any length.
  \item \verb|\alph{foo}| produces \alph{foo}
\end{itemize}




